Sampling-based Reactive Synthesis for Nondeterministic Hybrid Systems

This paper introduces a sampling-based strategy synthesis algorithm for nondeterministic hybrid systems with complex continuous dynamics under temporal and reachability constraints. We model the evolution of the hybrid system as a two-player game, where the nondeterminism is an adversarial player whose objective is to prevent achieving temporal and reachability goals. The aim is to synthesize a winning strategy -- a reactive (robust) strategy that guarantees the satisfaction of the goals under all possible moves of the adversarial player. Our proposed approach involves growing a (search) game-tree in the hybrid space by combining sampling-based motion planning with a novel bandit-based technique to select and improve on partial strategies. We show that the algorithm is probabilistically complete, i.e., the algorithm will asymptotically almost surely find a winning strategy, if one exists. The case studies and benchmark results show that our algorithm is general and effective, and consistently outperforms state of the art algorithms.

==> sections/Extended/Experiments.tex <==
%  \begin{figure*}
%     \centering
%     \begin{subfigure}{0.23\textwidth}
%     \includegraphics[width=\textwidth, trim={4cm 6cm 4cm 6cm},clip]{figures/clutter.pdf}
%     \vspace{-7mm}
%     \caption{Cluttered}
%     \label{fig:clutter}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.23\textwidth}
%     \includegraphics[width=\textwidth, trim={4cm 6cm 4cm 6cm},clip]{figures/narrow.pdf}
%     \vspace{-7mm}
%     \caption{Narrow Passage}
%     \label{fig:narrow}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.23\textwidth}
%     \includegraphics[width=\textwidth, trim={4cm 6cm 4cm 6cm},clip]{figures/reallynarrow.pdf}
%     \vspace{-7mm}
%     \caption{Very Narrow Passage}
%     \label{fig:reallynarrow}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.23\textwidth}
%     \includegraphics[width=\textwidth, trim={4cm 6cm 4cm 6cm},clip]{figures/maze.pdf}
%     \vspace{-7mm}
%     \caption{Maze}
%     \label{fig:maze}
%     \end{subfigure}
% \caption{Four environments for benchmarking. Initial position and goal region are shown as blue and green circles, respectively.}
% \label{fig:benchmark environments}
% \vspace{-3.5mm}
% \end{figure*}

% \begin{table*}[!ht]
%     \centering
%     \caption{\small Benchmark planner performance results. We report the mean time with standard error, and success rate over 100 simulation trials, with best scores in bold. RRT in case study 2 and MCTS for both cases are excluded from the table since they had $0$ success rate.}
%     \label{tab:benchmarks}
%     \scalebox{0.94}{
%     \begin{tabular}{c c c c c c c c c c}
%     \toprule
%     & \multirow{2}{*}{Algorithm}&  \multicolumn{2}{c}{\underline{\hspace{7mm} Environment 1 \hspace{7mm}}} & \multicolumn{2}{c}{\underline{\hspace{7mm} Environment 2 \hspace{7mm}}} & \multicolumn{2}{c}{\underline{\hspace{7mm} Environment 3 \hspace{7mm}}} & \multicolumn{2}{c}{\underline{\hspace{7mm} Environment 4 \hspace{7mm}}}\\
%     &  & Time (s)& Success  (\%) & 
%     Time (s)& Success (\%) & Time (s)& Success  (\%) & Time  & Success  (\%)\\
%     \hline
%      % \multicolumn{9}{|c|}{Case Study 1}\\
%      \multirow{3}{*}{Case 1} & RRT   & $299.0 \pm 0.0$ & $3$  & $299.5 \pm 0.0$ &  $2$  & $300 \pm 0.0$  &  $1$ & -  & $0$ \\
%      & Planner in \cite{Lahijanian2014} & $78.1 \pm 4.6$ & $91$ & $113.1 \pm 9.1$ & 82 & $153.68 \pm 15.5$ & $44$ & $222.5 \pm 26.3$ & $10$ \\
%      & SaBRS  (Ours) & $\mathbf{4.2 \pm 0.5}$ & $\mathbf{100}$ & $\mathbf{8.3 \pm 1.1}$ & $\mathbf{100}$ & $\mathbf{23.04 \pm 3.6}$ & $\mathbf{99}$ & $\mathbf{57.9 \pm 6.5}$ & $\mathbf{93}$ \\
%      \hline
%      % \multicolumn{9}{|c|}{Case Study 2}\\\hline
%      \multirow{2}{*}{Case 2}  & Planner in \cite{Lahijanian2014} & $98.1 \pm 6.5$ & 96 & $157.1 \pm 12.0$ & $68$ & $208.9 \pm 18.3$ & $32$ & $251.1 \pm 49.0$ & $4$ \\
%      % \hline
%     & SaBRS (Ours) & $\mathbf{4.6 \pm 0.5}$ & $\mathbf{100}$ & $\mathbf{11.4 \pm 2.8}$ & $\mathbf{99}$ & $\mathbf{24.4 \pm 4.0}$ & $\mathbf{97}$ & $\mathbf{48.99 \pm 6.8}$ & $\mathbf{88}$\\
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{-4mm}
% \end{table*}


\section{Experiments}

We evaluate the performance of SaBRS against state-of-the-art algorithms RRT planner, a continuous space MCTS algorithm (MCTS-PW), and the nondeterministic motion planner in \cite{Lahijanian2014} in a series of benchmarks. We also provide several illustrative examples to show the generality of SaBRS. We implement all algorithms in \texttt{C++} using OMPL \cite{sucan2012the-open-motion-planning-library}.  All computations are performed single-threaded on a nominally 3.60 GHz CPU with 32 GB RAM.


% Note that for a general NHS, it can be difficult to design a node evaluation heuristic for a hybrid space since distance over both discrete and continuous components can be difficult to define, and is an active area of research \cite{partialsatisfactionhybridsystem}.

\subsection{Benchmarking Results}

We first evaluate the algorithms on the benchmark problems proposed in \cite{Lahijanian2014}.  
The problems consists of two NHS models of a three-gear second-order car system that is subject to nondeterminism when shifting gears in the four environments considered in \cite{Lahijanian2014}.
% In the first case study, we consider a three-gear second-order car system which is subject to nondeterminism when shifting from gear two to three. 
In Case Study $1$, the system, when shifting from gear two to three, may mistakenly change to gear one instead of three. In Case Study $2$, there is an additional nondeterminism when the car has to shift from gear three to one. In this case, the system may mistakenly change to gear two instead of one. We refer the reader to \cite{Lahijanian2014} for details on the dynamics of each gear.

 We provided a time limit of $300$ seconds  to find a solution for 100 trials for each of the four environments and two cases. The results are summarized in Table~\ref{tab:benchmarks}. For the first case study, MCTS did not find any solutions. For the second case study, both RRT and MCTS did not find any solutions. It is evident from the poor performance of both RRT and MCTS that neither a purely sampling-based exploration method nor a purely heuristic search method works for finding winning strategies for NHS planning problems. Additionally, we see that SaBRS significantly outperforms the compared methods both in computation time (up to an order of magnitude) and success rate (up to 3$\times$) of finding winning strategies. This suggests that the combination of the bandit-based game theoretic approach for strategy selection and sampling-based exploration is important for reactive synthesis under nondeterministic uncertainty.

% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%     \hline
%     & \multicolumn{2}{c|}{Environment 1} & \multicolumn{2}{c|}{Environment 2} & \multicolumn{2}{c|}{Environment 3} & \multicolumn{2}{c|}{Environment 4}\\
%     \hline
%     Algorithm & Time (s)& Success (\%) & 
%     Time (s)& Success (\%) & Time (s)& Success (\%) & Time (s)& Success (\%)\\
%     \hline
%      \multicolumn{9}{|c|}{Case Study 1}\\
%     \hline
%      RRT   & $299.0$ & $3$  & $299.5$ &  $2$  & $300 \pm$  &  $1$ & -  & $0$ \\\hline
%      MCTS & $-$ & $-$  & $-$ &  $-$  & $-$  &  $-$ & -  & $-$ \\\hline
%      \cite{Lahijanian2014} & 75.0581 & 91 & 113.05 & 82 & 153.68 & 44 & 222.5 & 10 \\\hline
%      Ours & 4.175 & 100 & 8.334 & 100 & 23.04 & 99 & 57.89 \\
%      \hline
%      \multicolumn{9}{|c|}{Case Study 2}\\\hline
%      RRT    & - & 0 & - & 0 & - & 0 & - & 0  \\\hline
%      MCTS& - & 0 & - & 0 & - & 0 & - & 0  \\\hline
%      \cite{Lahijanian2014} & 98.1239 & 96 & 157.14 & 68 & 208.88 & 32 & 251.1 & 4 \\\hline
%      Ours & 4.6185 & 100 & 11.377 & 99 & 24.42 & 97 & 48.99 & 88\\\hline
%     \end{tabular}
%     \caption{\small Benchmark planner performance results. Each entry is the mean of 100 simulations.}
%     \label{tab:benchmarks}
%     \vspace{-4mm}
% \end{table*}

\subsection{Robotic Charging System}

Next, we showcase SaBRS's versatility to handle NHS with time constraints. Consider a robot with second-order car dynamics with a bounded motion disturbance at every time step, which is equipped with a closed-loop controller that is able to maintain the robot in a ball of radius $r$ around its nominal plan. 

The robot is tasked with navigating to the charger within $2$ minutes. If it goes over a water puddle, the robot needs to dry off on the carpet for $10$ seconds before going to the charger. Online, robot has perfect observation of its state. However, during offline planning, due to the motion disturbance, if the radius $r$ ball around a nominal plan intersects with a water puddle, the robot may traverse the puddle during execution. Figs. ~\ref{fig:waterpuddle1} and \ref{fig:waterpuddle2} show two examples with different obstacle configurations. In both cases, SaBRS finds a solution within $30$ seconds. In Fig.~\ref{fig:waterpuddle1}, when there is more space for the robot to traverse in the dry regions (in white), SaBRS synthesizes a strategy such that the entire ball stays within the white region without touching the water (in blue) and navigates to the charger (green). When the environment is more cluttered (Fig.~\ref{fig:waterpuddle2}), such that the robot cannot reach the charger without guaranteeing that it does not go over the water puddle due to the uncertain ball, SaBRS plans a reactive strategy with two possible trajectories. If it does not get wet, it navigates directly to the charger. If it gets wet, it first goes to and stays on the carpet for $10$ seconds before navigating to the charger.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.5\textwidth}
    \includegraphics[width=\textwidth, trim={3cm 10cm 3cm 10cm},clip]{figures/carpet_nosplit.pdf}
        % \vspace{-1mm}
    \caption{\small Spaced Obstacles}
    \label{fig:waterpuddle1}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
    \includegraphics[width=\textwidth, trim={3cm 10cm 3cm 10cm},clip]{figures/carpet_split.pdf}
    % \vspace{-1mm}
    \caption{\small Cluttered Obstacles}
    \label{fig:waterpuddle2}
    \end{subfigure}
\caption{\small Robotic charging example with different obstacle (in black) configuration. The blue, grey and green regions represents the puddle, carpet, and charger, respectively. SaBRS synthesizes a strategy that accounts for nondeterminism in traversing the puddle due to motion uncertainty.}
\label{fig:puddle}
\vspace{-3mm}
\end{figure}

\subsection{Search-and-rescue Scenarios}

Finally, we show that SaBRS is general and effective for problems with complex temporal specifications. We consider variants of the search-and-rescue scenario of Example~\ref{ex:searchandrescue}. The variants are:

\begin{enumerate}
    \item \textbf{Scenario 1}: All doors are known to be open, human location is unknown.
    \item \textbf{Scenario 2}: The door to room one is unknown, the door to room two is known to be open, and human location is unknown.
    \item \textbf{Scenario 3}: The door to room one is known to be open, the door to room two is unknown, and human location is unknown.
    \item \textbf{Scenario 4}: Door states are unknown, and human location is unknown.
    \item \textbf{Scenario 5}: Door states are unknown, but human is either in room one or two (never in room three).
\end{enumerate}

For each scenario, we provided SaBRS $20$ seconds to compute a solution. Figs~\ref{fig:searchandrescue_trajectories1}-\ref{fig:searchandrescue_trajectories5} show example synthesized strategies for each scenario. A room is considered searched if the robot enters a purple region, and the door (possibly open) of a room is depicted in gray. Each possible trajectory in the reactive strategy is plotted with a different color, and where a red dotted path segment indicates a nondeterministic mode transition. SaBRS successfully finds a winning strategy for each scenario that reacts based on if a door is open or closed, and if the human is possibly in each room.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth, trim={14.75cm 2.75cm 12.5cm 2.25cm},clip]{figures/searchandrescue_trajectories_scenario1.png}
    \caption{\small Example synthesized strategy for building search-and-rescue example, scenario 1.}
    \label{fig:searchandrescue_trajectories1}
    \vspace{-3mm}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth, trim={14.75cm 2.75cm 12.5cm 2.25cm},clip]{figures/searchandrescue_trajectories_scenario2.png}
    \caption{\small Example synthesized strategy for building search-and-rescue example, scenario 2.}
    \label{fig:searchandrescue_trajectories2}
    \vspace{-3mm}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth, trim={14.75cm 2.75cm 12.5cm 2.25cm},clip]{figures/searchandrescue_trajectories_scenario3_3.png}
    \caption{\small Example synthesized strategy for building search-and-rescue example, scenario 3.}
    \label{fig:searchandrescue_trajectories3}
    \vspace{-1mm}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth, trim={14.75cm 2.75cm 12.5cm 2.25cm},clip]{figures/searchandrescue_trajectories.png}
    \caption{\small Example synthesized strategy for building search-and-rescue example, scenario 4.}
    \label{fig:searchandrescue_trajectories4}
    \vspace{-3mm}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth, trim={14.75cm 2.75cm 12.5cm 2.25cm},clip]{figures/searchandrescue_trajectories_scenario5.png}
    \caption{\small Example synthesized strategy for building search-and-rescue example, scenario 5.}
    \label{fig:searchandrescue_trajectories5}
    \vspace{-3mm}
\end{figure}
